Quantitative comparison of opacities calculated using the $R$-matrix and Distorted-Wave methods: Fe XVII

We present here a detailed calculation of opacities for Fe~XVII at the physical conditions corresponding to the base of the Solar convection zone. Many ingredients are involved in the calculation of opacities. We review the impact of each ingredient on the final monochromatic and mean opacities (Rosseland and Planck). The necessary atomic data were calculated with the $R$-matrix and the distorted-wave (DW) methods. We study the effect of broadening, of resolution, of the extent of configuration sets and of configuration interaction to understand the differences between several theoretical predictions as well as the existing large disagreement with measurements. New Dirac $R$-matrix calculations including all configurations up to the $n=$ 4, 5 and $6$ complexes have been performed as well as corresponding Breit--Pauli DW calculations. The DW calculations have been extended to include autoionizing initial levels. A quantitative contrast is made between comparable DW and $R$-matrix models. We have reached self-convergence with $n=6$ $R$-matrix and DW calculations. Populations in autoionizing initial levels contribute significantly to the opacities and should not be neglected. The $R$-matrix and DW results are consistent under the similar treatment of resonance broadening. The comparison with the experiment shows a persistent difference in the continuum while the filling of the windows shows some improvement. The present study defines our path to the next generation of opacities and opacity tables for stellar modeling.

==> IonicState.tex <==
\begin {table}[H]
\caption {Ionic fractions as a function of $FeXVII$ models} \label{tab:IonPop} 
begin{tabular}{ l l l l l }
   $FeXVII$ Model & $Fe XX$ & $Fe XIX$ & $Fe XVIII$ & $Fe XVII$ \\
   OPCD 2005 & $1.0273 \times 10^{-1}$ &  $2.9913 \times 10^{-1}$  & $3.9200 \times 10^{-1}$   & $2.0614 \times 10^{-1}$  \\
   $R-matrix$ n=4 74 levels in $Fe XVII$ & $1.0273 \times 10^{-1}$ &  $2.9913 \times 10^{-1}$  & $3.9200 \times 10^{-1}$   & $2.0614 \times 10^{-1}$  \\
   $R-matrix$ n=5 132 levels in $Fe XVII$ & $1.0273 \times 10^{-1}$ &  $2.9913 \times 10^{-1}$  & $3.9200 \times 10^{-1}$   & $2.0614 \times 10^{-1}$  \\
   $R-matrix$ n=6 328 levels in $Fe XVII$ & $1.0273 \times 10^{-1}$ &  $2.9913 \times 10^{-1}$  & $3.9200 \times 10^{-1}$   & $2.0614 \times 10^{-1}$  \\
 \end{tabular}
\caption {Variation of the ion populations depending on the model of $FeVII$ used. The differences come from the diferent first ionization thresholds as
well as from the number of levels present in the $FeXVII$ model.}
\end{center}
\end {table}

